Validation of the $^{10}\mathrm{Be}$ Ground-State Molecular Structure Using $^{10}\mathrm{Be}(p,p\alpha)^{6}\mathrm{He}$ Triple Differential Reaction Cross-Section Measurements

The cluster structure of the neutron-rich isotope $^{10}$Be has been probed via the $(p,p\alpha)$ reaction at 150 MeV/nucleon in inverse kinematics and in quasifree conditions. The populated states of $^{6}$He residues were investigated through missing mass spectroscopy. The triple differential cross-section for the ground-state transition was extracted for quasifree angle pairs ($\theta_{p}$, $\theta_{\alpha}$) and compared to distorted-wave impulse approximation reaction calculations performed in a microscopic framework using successively the Tohsaki-Horiuchi-Schuck-R\"opke product wave-function and the wave-function deduced from Antisymmetrized Molecular Dynamics calculations. The remarkable agreement between calculated and measured cross-sections in both shape and magnitude validates the molecular structure description of the $^{10}$Be ground-state, configured as an $\alpha$-$\alpha$ core with two valence neutrons occupying $\pi$-type molecular orbitals.

==> sub/discussion.tex <==
\section{Discussions}
% Interpreted by Theory

